Exploring the total Galactic extinction with SDSS BHB stars

Aims: We used 12,530 photometrically-selected blue horizontal branch (BHB) stars from the Sloan Digital Sky Survey (SDSS) to estimate the total extinction of the Milky Way at the high Galactic latitudes, $R_V$ and $A_V$ in each line of sight. Methods: A Bayesian method was developed to estimate the reddening values in the given lines of sight. Based on the most likely values of reddening in multiple colors, we were able to derive the values of $R_V$ and $A_V$. Results: We selected 94 zero-reddened BHB stars from seven globular clusters as the template. The reddening in the four SDSS colors for the northern Galactic cap were estimated by comparing the field BHB stars with the template stars. The accuracy of this estimation is around 0.01\,mag for most lines of sight. We also obtained $<R_V>$ to be around 2.40$\pm1.05$ and $A_V$ map within an uncertainty of 0.1\,mag. The results, including reddening values in the four SDSS colors, $A_V$, and $R_V$ in each line of sight, are released on line. In this work, we employ an up-to-date parallel technique on GPU card to overcome time-consuming computations. We plan to release online the C++ CUDA code used for this analysis. Conclusions: The extinction map derived from BHB stars is highly consistent with that from Schlegel, Finkbeiner & Davis(1998). The derived $R_V$ is around 2.40$\pm1.05$. The contamination probably makes the $R_V$ be larger.

==> figs_pdf.tex <==
\clearpage

\begin{figure*}
\epsscale{1.0}
\plotone{fig/Color_Mg-eps-converted-to.pdf}
\caption{The 94 dereddened BHB stars and two typical isochrones in the  color vs. absolute magnitude plane. The blue points are the BHB stars, the green curve is the isochrone with metallicity of -2.28\,dex and age of 13.5\,Gyrs. And the red curve is another isochrone with metallicity -2.0 at same age. Both isochrones are obtained from \citet{girardi10}. 
\label{Color_Mg}}
\end{figure*}


\begin{figure*}
\epsscale{1.5}
\plotone{fig/simu1.pdf}
\caption{One \textbf{simulated \los} example of 900 Monte Carlo simulations for validation of Bayesian method. In the left panel, the blue crosses stands for the 94 template BHB stars, the red points are selected \textbf{field} stars with random reddening values and random Gaussian noises in photometry. The right panel shows the contour of the posterior probability of the reddening $E(u-g)$ and $E(g-r)$ estimated from the Bayesian method. The large blue cross marks the most-likely reddening values with $1\sigma$ error.
\label{fig_simu1}}
\end{figure*}


\begin{figure*}
\epsscale{1.5}
\plotone{fig/simu_comparing-eps-converted-to.pdf}
\caption{The estimated reddening values versus the given values in the simulation. The mean 1$\sigma$ error bars are marked at the bottom.
\label{fig_simu_comparing}}
\end{figure*}

\begin{figure*}
\epsscale{1.0}
\plotone{fig/simu_E_contrast-eps-converted-to.pdf}
\caption{ Histogram of the residuals of the estimated reddening values in the simulation. The red curves are the Gaussian fit profiles with $\sigma \simeq 0.01$.
\label{fig_simu_contrast}}
\end{figure*}

\begin{figure*}
\epsscale{0.6}
\plotone{fig/hist_RV_SDSS_simu-eps-converted-to.pdf}
\caption{Histogram of estimated $R_V$ in the simulation. \textbf{The red curves are the Gaussian fit profiles with the mean value $<R_V> \simeq 3.1$, and $\sigma \simeq 0.16$, the yellow line marks the location of $R_V = 3.1$}. \label{Rv_Hist_sim}}
\end{figure*}


\begin{figure*}
\epsscale{1.2}
\plotone{fig/data_distr-eps-converted-to.pdf}
\caption{Data sample distribution. The black points are the 13,143 BHB candidates selected in this work. We confirm that these samples are contaminated by at least 76 Main sequence stars (red circles), 311 Blue Straggler (green points), and 227 other objects(yellow points)\citep{xue08}. The 7 globular star clusters listed in the Table \ref{tbl-1} are marked by blue circles.\label{fig_data}}
\end{figure*}


\begin{figure*}
\epsscale{1.6}
\plotone{fig/2color-eps-converted-to.pdf}
\caption{The panels show all of the BHB stars used in this work in the color-color space. The tails of black points are due to the extinction. The red points are the 94 template BHB stars, which are calibrated with the known extinction. The magenta arrows present the reddening direction, the starting point of each arrow is the median value of the color indexes of the 94 template stars, and the terminal is the reddened original point with $R_V = 3.1$ and $E(B-V)=0.1$.
\label{fig_data_color}}
\end{figure*}

\begin{figure*}
\centering 
\epsscale{3.0}
\plottwo{fig/Eugmap_eq.eps}{fig/Egrmap_eq-eps-converted-to.pdf}
\caption{The reddening maps for $E(u-g)$ (top panel) and $E(g-r)$ (bottom panel). The top plots in each panel give the reddening map estimated by the Bayesian method, while the bottom ones show the same map released by SDSS. \textbf{The blanks and other features in our maps are probably because that the reddening values are too smaller in the high galactic latitude to be estimated accurately, the reddening values in these regions are very close to the average of photometric error}. 
\label{fig_reddening_ugr}}
\end{figure*}

\begin{figure*}
\centering 
\epsscale{3.0}
\plottwo{fig/Erimap_eq.eps}{fig/Eizmap_eq-eps-converted-to.pdf}
\caption{The reddening maps for $E(r-i)$ (top panel) and $E(i-z)$ (bottom panel). The top plots in each panel give the reddening map estimated by the Bayesian method, while the bottom ones show the same map released by SDSS.
\label{fig_reddening_riz}}
\end{figure*}

\begin{figure*}
\centering 
\epsscale{1.5}
\plotone{fig/Avmap_eq-eps-converted-to.pdf}
\caption{The top panel shows the $A_V$ map, while the bottom \textbf{panel} shows its error in same color level, \textbf{the value of $A_V$ is the median $A_V$ of all the BHB stars in each \los, and the error is calculated by the median absolute deviation of $A_V$ in each \los}. \label{Rv_Av_Map}}
\end{figure*}

\begin{figure*}
\epsscale{1.5}
\plotone{fig/Glat_Rv_hist3-eps-converted-to.pdf}
\caption{The distribution of the estimated $R_V$ is shown in the left panel. The red line shows the best fit Gaussian with $\mu\simeq 2.4$ and $\sigma\simeq 1.05$. The middle and right panels are the estimated $R_V$ as function of Galactic latitude and longitude, respectively. The red curves show the $<R_V>$, which keeps constant at $\sim 2.5$ over all latitudes and longitudes.\label{Rv_Hist}
}
\end{figure*}


\begin{figure*}
\epsscale{1.6}
\plotone{fig/2color_contamination_ra237_dec24-eps-converted-to.pdf}
\caption{Color-Color diagrams of the 18 BHB stars(black circles) on the \los\ of $(l, b) =(39, 50)$, and 24 contamination stars (blue points) on this \los, selected from \cite{smith2010}. The magenta arrows present the reddening direction, the starting point of each arrow is the median value of the color indexes of the 18 field stars, and the terminal is the reddened original point with $R_V = 3.1$ and $E(B-V)=0.1$. 
\label{2color_contami}}
\end{figure*}

%\begin{figure*}
%\epsscale{1.6}
%\plotone{fig/Eugriz_Rv-eps-converted-to.pdf}
%\caption{This Diagram shows how the $R_V$ varies with the ratios of the reddening in the different colors. It is drawn according to the Eq. \ref{Extinc}. As the increasing of $E(u-g)/E(g-r)$, the $R_V$ tends to be smaller. The simulation indicates that the contaminations make the $E(u-g)$ drop much more seriously relative to the $E(g-r)$, which is probably one of reasons why our $R_V$ measured in this works is smaller than the most frequently used value of 3.1.
%\label{Eugriz_Rv}}
%\end{figure*}

\begin{figure*}
\epsscale{4.0}
\plottwo{fig/Glat_delta_E1.eps}{fig/Glat_delta_E2-eps-converted-to.pdf}
\caption{The blue dots are the differences between the estimated reddening in this work and those from SDSS at different Galactic latitude.  The green lines indicate $\Delta E(a-b)=0$ and the red curves the average values of the differential reddening values in different Galactic latitude bins.
\label{fig_contrast_reddening1}}
\end{figure*}
